Domain Adaptation for Semantic Segmentation via Patch-Wise Contrastive Learning

We introduce a novel approach to unsupervised and semi-supervised domain adaptation for semantic segmentation. Unlike many earlier methods that rely on adversarial learning for feature alignment, we leverage contrastive learning to bridge the domain gap by aligning the features of structurally similar label patches across domains. As a result, the networks are easier to train and deliver better performance. Our approach consistently outperforms state-of-the-art unsupervised and semi-supervised methods on two challenging domain adaptive segmentation tasks, particularly with a small number of target domain annotations. It can also be naturally extended to weakly-supervised domain adaptation, where only a minor drop in accuracy can save up to 75% of annotation cost.

==> fig/impact.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{figure*}
\centering
\includegraphics[width=1.0\linewidth,height=5.5cm]{images/impact.pdf}
\vspace{-6mm}
\caption{{\small \bf Impact by Target Domain Labels.} Dashed lines represent UDA approaches while solid lines are SSDA.}
\label{fig:impact}
\end{figure*}

==> table/weak.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{table}
  \centering
    \begin{tabular}{cc}
  \toprule
  Annotation Rate & mIoU \\
  \midrule
 $100\%$ & {\bf 56.96}  \\
 \midrule
 $75\%$ & 56.68  \\
 $50\%$ & 56.21 \\
 $25\%$ &55.94 \\
  \bottomrule
  \end{tabular}
  \caption{ {\bf Quantitative Comparison of Weak Annotation.} We evaluate our approach with 200 labelled target domain images and different annotation rate, as the table shows, our approach compatible with block annotations which still get competing performance with much less annotated blocks.}
  \label{tab:weak}
\end{table}
